Panoptic SegFormer: Delving Deeper into Panoptic Segmentation with Transformers

Panoptic segmentation involves a combination of joint semantic segmentation and instance segmentation, where image contents are divided into two types: things and stuff. We present Panoptic SegFormer, a general framework for panoptic segmentation with transformers. It contains three innovative components: an efficient deeply-supervised mask decoder, a query decoupling strategy, and an improved post-processing method. We also use Deformable DETR to efficiently process multi-scale features, which is a fast and efficient version of DETR. Specifically, we supervise the attention modules in the mask decoder in a layer-wise manner. This deep supervision strategy lets the attention modules quickly focus on meaningful semantic regions. It improves performance and reduces the number of required training epochs by half compared to Deformable DETR. Our query decoupling strategy decouples the responsibilities of the query set and avoids mutual interference between things and stuff. In addition, our post-processing strategy improves performance without additional costs by jointly considering classification and segmentation qualities to resolve conflicting mask overlaps. Our approach increases the accuracy 6.2\% PQ over the baseline DETR model. Panoptic SegFormer achieves state-of-the-art results on COCO test-dev with 56.2\% PQ. It also shows stronger zero-shot robustness over existing methods. The code is released at \url{https://github.com/zhiqi-li/Panoptic-SegFormer}.

==> table/attnmaps.tex <==
\begin{tabular}{  c  c | c | c|  c|  c| c |c |c| c}
    \hline
    \multirow{2}{2cm}{Ground \\Truth} & \multirow{2}{2cm}{predicted \\result} &  \multicolumn{8}{c}{multi-head attention maps} \\
     & & 1& 2 & 3 & 4 & 5 & 6 & 7 & 8  \\ 
     \\
     
    \hline
    \begin{minipage}[b]{0.1\linewidth}
		\centering
	        {\includegraphics[width=\linewidth,height=4\linewidth]{media/visual/mask.pdf}}
	        \end{minipage}
    & 
    \begin{minipage}[b]{0.1\linewidth}
		\centering
		{\includegraphics[width=\linewidth,height=4\linewidth]{media/visual/predict.pdf}}
	\end{minipage}
	&
	\multicolumn{8}{c}{
	\begin{minipage}[b]{0.7\linewidth}
		\centering
		{\includegraphics[width=\linewidth,height=0.57\linewidth]{media/visual/attnmaps.pdf}}
	\end{minipage}
	}\\

  \end{tabular}

==> table/complexity.tex <==
\begin{tabular}{l|c|c|c|c|c }
\hline
Method & Backbone &  \#Param & FLOPs& Fps & Memory \\
\hline
Deformable DETR*\cite{mmdetection,zhu2020deformable} & R50&39.8M & 195G & 15& 4567M \\
\hline
Panoptic SegFormer & R50&  47.0M & 246G & 13& 7722M\\
Panoptic SegFormer & R101&  65.9M & 322G & 10 & 8396M\\
Panoptic SegFormer & PVTv2-B5& 100.9M & 391G & 5 &23112M \\
\hline

\end{tabular}

==> table/deformable.tex <==


%\begin{tabular}[b]{l| p{1.2cm}<{\centering}| p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}|p{1cm}<{\centering}p{1cm}<{\centering}p{1cm}<{\centering}}
	% \whline

%	&  &\multicolumn{3}{c|}{Panoptic Segmentation} & \multicolumn{3}{c}{Object Detection}\\
	%Method& Epoch& PQ & PQ$^{\rm th}$ & RQ$^{\rm st}$ & AP & AP$_{\rm 50}$ & AP$_{\rm 75}$ \\
	%\hline
	%DETR~\cite{carion2020end} & 500 &43.4 & 48.2 & 36.3 & 42.0 & 62.4 & 44.2\\
    %D-DETR-SS*~\cite{zhu2020deformable} &50 & 40.6 &44.0 & 35.4 &39.4 &59.6&42.3\\
    %D-DETR-MS*~\cite{zhu2020deformable} & 50 & 45.4 &50.0 &38.5 &44.5	 & 63.6&48.7\\

%\end{tabular}
\begin{tabular}[b]{l| c|c c c}
	% \whline
	%&  &\multicolumn{3}{c|}{Panoptic Segmentation} \\
	Method& Epoch& PQ & PQ$^{\rm th}$ & PQ$^{\rm st}$  \\
	\hline
	DETR~\cite{carion2020end} & 500 &43.4 & 48.2 &36.3\\
    D-DETR-SS*~\cite{zhu2020deformable} &50 & 40.6 &44.0 & 35.4 \\
    D-DETR-MS*~\cite{zhu2020deformable} &50 & 46.3 &51.9 &37.9 \\

\end{tabular}




==> table/ds2.tex <==
\begin{tabular}{c c  c }

    & w/ deep-sup & w/o deep-sup \\
    \rotatebox{90}{layer1}
    &
    \begin{minipage}[b]{0.4\linewidth}
		\centering
	        {\includegraphics[width=\linewidth]{media/ds/ds0.pdf}}
	        \end{minipage}
    & 
    \begin{minipage}[b]{0.4\linewidth}
		\centering
		{\includegraphics[width=\linewidth]{media/ds/nds0.pdf}}
	\end{minipage}
	\\
	\rotatebox{90}{layer3}
    &
    \begin{minipage}[b]{0.4\linewidth}
		\centering
	        {\includegraphics[width=\linewidth]{media/ds/ds1.pdf}}
	        \end{minipage}
    & 
    \begin{minipage}[b]{0.4\linewidth}
		\centering
		{\includegraphics[width=\linewidth]{media/ds/nds1.pdf}}
	\end{minipage}
	\\
	\rotatebox{90}{layer6}
    &
    \begin{minipage}[b]{0.4\linewidth}
		\centering
	        {\includegraphics[width=\linewidth]{media/ds/ds4.pdf}}
	        \end{minipage}
    & 
    \begin{minipage}[b]{0.4\linewidth}
		\centering
		{\includegraphics[width=\linewidth]{media/ds/nds4.pdf}}
	\end{minipage}
	\\
	\rotatebox{90}{result}
    &
    \begin{minipage}[b]{0.4\linewidth}
		\centering
	        {\includegraphics[width=\linewidth]{media/ds/ds.pdf}}
	        \end{minipage}
    & 
    \begin{minipage}[b]{0.4\linewidth}
		\centering
		{\includegraphics[width=\linewidth]{media/ds/nds.pdf}}
	\end{minipage}
	
	
  
	%\hline
  \end{tabular}

==> table/query.tex <==
\begin{tabular}{l c  c c  }
\toprule
Method &  \#Query & PQ & PQ$^{\rm st}$ \\
\midrule
Joint Matching & 353 &  48.5  &39.5 \\
Query Decoupling & 300+53 & 49.6& 42.4\\
\bottomrule
\end{tabular}

==> table/schedule.tex <==
\begin{tabular}{p{3cm}|p{1.6cm}<{\centering}|p{0.8cm}<{\centering} p{0.8cm}<{\centering}p{0.8cm}<{\centering}  }

Method &  \#Query & PQ & PQ$^{\rm th}$ &  PQ$^{\rm st}$ \\
\hline
Joint Matching& 353 &  46.1 & 52.6 &36.3 \\
Separate Matching & 300+53 & 47.0 & 52.3& 38.9 \\
Query Decoupling & 300+53 & 48.0& 52.3& 41.5\\

\end{tabular}
